AdaTriplet: Adaptive Gradient Triplet Loss with Automatic Margin Learning for Forensic Medical Image Matching

This paper tackles the challenge of forensic medical image matching (FMIM) using deep neural networks (DNNs). FMIM is a particular case of content-based image retrieval (CBIR). The main challenge in FMIM compared to the general case of CBIR, is that the subject to whom a query image belongs may be affected by aging and progressive degenerative disorders, making it difficult to match data on a subject level. CBIR with DNNs is generally solved by minimizing a ranking loss, such as Triplet loss (TL), computed on image representations extracted by a DNN from the original data. TL, in particular, operates on triplets: anchor, positive (similar to anchor) and negative (dissimilar to anchor). Although TL has been shown to perform well in many CBIR tasks, it still has limitations, which we identify and analyze in this work. In this paper, we introduce (i) the AdaTriplet loss -- an extension of TL whose gradients adapt to different difficulty levels of negative samples, and (ii) the AutoMargin method -- a technique to adjust hyperparameters of margin-based losses such as TL and our proposed loss dynamically. Our results are evaluated on two large-scale benchmarks for FMIM based on the Osteoarthritis Initiative and Chest X-ray-14 datasets. The codes allowing replication of this study have been made publicly available at \url{https://github.com/Oulu-IMEDS/AdaTriplet}.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> aleksei.tex <==
\section{Aleksei's sandbox}
We consider a setting of image retrieval, and optimize the triplet loss:
\begin{equation}
    \mathcal{L}_{\mathrm{trip}} = \max\left( \| f_\theta(x_a) - f_\theta(x_p) \right \|_2^2 - \left \| f_\theta(x_a) - f_\theta(x_n) \|_2^2 + \epsilon, 0 \right),
    \label{eq:triplet_loss}
\end{equation}
where $\epsilon$ is a margin variable that needs to be chosen empirically. We call a case positive if the patient's identities match. Our contribution is to add the following regularizer to the triplet loss:
\begin{align}
    \max(f_\theta(x_a)^\intercal f_\theta(x_n) + \beta, 0),
\end{align}
where $m_n$ is another margin. So, finally, we want to solve:
\begin{equation}
    \hat \theta = \arg\min_\theta \left[\mathcal{L}_{\mathrm{trip}} + \max\left( f_\theta(x_a)^\intercal f_\theta(x_n) + \beta, 0\right)\right].
    \label{eq:triplet_loss}
\end{equation}
\subsection{Questions to resolve / action points}
\begin{enumerate}
    \item Clean up the math.
    \item How do state-of-the-art losses perform?  (we may not need to check this, as there is a paper by Kevin Musgrave showing that there is actually no improvement by SOTA over contrastive or triplet losses).
    %\item How about then taking the following alternative to the triplet loss (note that degree of the anchor-negative distance has been downgraded):
    %\begin{align}
    %    \mathcal{L}_{\mathrm{trip}} = \max\left( \| f_\theta(x_a) - f_\theta(x_p) \right \|_2^2 - \left \| f_\theta(x_a) - f_\theta(x_n) \|_2 + \epsilon, 0 \right),
    %\end{align}
    \item What is the effect of taking the regularizer as is vs taking the LSE upper bound?
    \item What is the effect of taking the LSE upper bound on triplet loss
    \item Some visualizations in 3D would help to understand the loss better!
    \item Try to tune $\beta$.
\end{enumerate}

\section{Aleksei's sandbox N2}
\begin{itemize}
    \item We are not happy with triplet loss, because it looks at the \textit{relative} difference between the angles (p-a and n-a)
    \item However, we argue that this loss forgets about driving representations between the anchor and the negative apart on themselves. When we achieve the margin, we stop learning (make a visualization). Make a code generated figure. 
    \item We drive representations apart using contrastive loss. 
    \item One can see that we can also drive representations together (anchor and positive), but it is not a good idea. 
    \item Have all the details written for dummies (like me) 
    \item Do not abuse the notation with extra symbols. No, it does not make your paper look better
\end{itemize}

==> khanh.tex <==
$N_P$ number of total labels \\
$n_p$ number of labels in vertical plane \\
$N_d$ number of vertical planes \\

$\alpha$ = angle between labels\\
We want to locate total labels in unit sphere in such way that each label is equidistant  with angle $\alpha$ in the same plane $D$, and plane $D$ is also equidistant each other with angle $\alpha$. \\
Denote
\begin{align}
    N_p &= n_p*N_d
\end{align}
2 planes crossed each other creates 2 angles $\alpha$. In one plane which is unit circle, from the center to different label has the same angle $\alpha$:
\begin{align}
    2*\alpha*N_d &= 2\pi \\
    \alpha*n_p &= 2\pi 
\end{align}

\begin{align}
    \alpha &= \frac{2\pi}{2N_d} = \frac{\pi}{N_d} \ (\mathrm{Horizontal})\\
    \alpha &= \frac{2\pi}{n_p} = \frac{2\pi}{\frac{N_P}{N_d}} = \frac{2\pi*N_d}{N_P} \ (\mathrm{Vertical})
\end{align}
from (4),(5)
\begin{align}
    \frac{2N_d}{N_P} &= \frac{1}{N_d} \\
    N_d &= \sqrt{\frac{N_P}{2}} \\
    n_p &= \frac{N_P}{N_d} = \frac{N_P}{\sqrt{\frac{N_P}{2}}} = \sqrt{2N_P}\\
    \alpha &= \frac{\pi*\sqrt{2}}{\sqrt{N_P}}
\end{align}
We realized, even each label is equidistant in plane, and plane is equidistant the same angle, there are several labels overlap on 2 polar of sphere. The reason is each plane crosses the sphere at the same points. We once again relocate overlaped label. Number of labels now become:
\begin{align}
    N_l &= 2(N_d -1)
\end{align}
Our data has large labels, also have large number of planes, so we can rewrite eq(11):
\begin{align}
    N_l &= 2*N_d
\end{align}
With the same idea, these labels needs to be equidistant each other with the angle $\beta$. Apply eq.(9):
\begin{align}
    \beta &= \frac{\pi*\sqrt{2}}{\sqrt{N_l}} 
    = \frac{\pi*\sqrt{2}}{\sqrt{2*N_d}}
    = \frac{\pi*\sqrt{2}}{\sqrt{2*\sqrt{\frac{N_P}{2}}}} 
    = \frac{\pi*\sqrt{2}}{\sqrt{\sqrt{2*N_P}}}
\end{align}
$\beta$ here is the different angle between 2 labels. For the $\beta$ used in our loss, rewrite as follows:
\begin{align}
      \beta &\ge 1-\frac{\pi*\sqrt{2}}{\sqrt{\sqrt{2*N_P}}}
\end{align}
For example $N_P=8$, $\alpha=\pi/2$, 2 points overlap, $\beta=\pi$ 







